ChemBO: Bayesian Optimization of Small Organic Molecules with Synthesizable Recommendations

In applications such as molecule design or drug discovery, it is desirable to have an algorithm which recommends new candidate molecules based on the results of past tests. These molecules first need to be synthesized and then tested for objective properties. We describe ChemBO, a Bayesian optimization framework for generating and optimizing organic molecules for desired molecular properties. While most existing data-driven methods for this problem do not account for sample efficiency or fail to enforce realistic constraints on synthesizability, our approach explores the synthesis graph in a sample-efficient way and produces synthesizable candidates. We implement ChemBO as a Gaussian process model and explore existing molecular kernels for it. Moreover, we propose a novel optimal-transport based distance and kernel that accounts for graphical information explicitly. In our experiments, we demonstrate the efficacy of the proposed approach on several molecular optimization problems.

==> ot_dist.tex <==


\section{An Optimal Transport Based Distance for Chemical Molecules}
\label{sec:otdist}

We now describe a distance $\otdistsymbol:\Xcal^2\rightarrow\RR_+$ between chemical
molecues. Given such a distance, we may use $\kernel = e^{-\beta \otdistsymbol}$,
where $\beta>0$, as the kernel.
We will assume some familiarity with concepts in chemistry such as bond types, and
atomic masses.
% 
To motivate this distance, note that the drug properties of a molecule is determined
not just by the atoms composing the molecules, but also their structure.
For example, both n-butane and isobutane have the same number of \chemmol{C} and
\chemmol{H} atoms (\chemmol{C\subscript{4}H\subscript{10}}), but have different chemical
properties due to different structure.
Hence, a distance should properly account for both these factors.
Following~\citet{kandasamy2018nasbot}, we will define this via a matching scheme
that attemps to match the atoms in one molecule to another.
The matching will only permit matching identical atoms, i.e. \chemmol{C} atoms can only
be matched to \chemmol{C} atoms, but we will incur penalties for matching atoms in
structurally dissimilar positions.
As we will see shortly, this matching scheme can be formulated as an optimal transport
(OT) program, which gives rise to efficient computation.

\insertFigOrganicEgs


\textbf{Chemical Molecules as Graphs:}
For what follows, it will be convenient to view a chemical molecule $M$ as a graph
$\molecule = (\atoms, \bonds)$, which is defined by a set of atoms $\atoms$ (vertices) and
a set of bonds $\bonds$ (edges).
A bond $(u, v)\in\bonds$ is an unordered pair of atoms $u, v\in\atoms$.
Each atom $a\in\atoms$ has a label, denoted $\atomlabel(a)$,
as does each bond $b\in\bonds$, denoted $\bondlabel(b)$.
For example, in our setting, $\atomlabel(a)$ could take values such as
\chemmol{C}, \chemmol{H}, or \chemmol{O}, indicating carbon, hydrogen, or oxygen atoms,
while
$\bondlabel(b)$ could take values such as
\singlebond, \doublebond, or \aromaticbond{}, indicating single, double, or
aromatic covalent bonds.
For example, in Figure~\ref{fig:organicegs}, atoms are represented by letters indicating
their label; bonds are represented by lines where single lines indicate single bonds and
double lines indicate double bonds.
% 
Next, we will assign weights $\atomwt(a)>0$ for all atoms
$a\in\atoms$ of a molecule ---
our matching scheme will attempt to match the weights in one molecule to another, in order
to compute a distance.
We will discuss choices for $\atomwt$ shortly.

We now describe our distance formulation.
Given two molecules $\molecule_1 = (\atoms_1, \bonds_1),
\molecule_2 = (\atoms_2, \bonds_2)$ with $n_1, n_2$ atoms respectively, 
we first let $Z\in\RR_+^{n_1\times n_2}$ be the matching matrix, i.e.
$Z(i,j)$ denotes the amount of weight matched between atom $i\in\molecule_1$ and
$j\in\molecule_2$.
The distance is then computed by solving the following linear program.
\begingroup
\allowdisplaybreaks
\begin{align*}
& \minimise_{Z}\quad \atomtypepen(Z) +
\structpen(Z) + \nonmatchpen(Z) 
\numberthis
\label{eqn:otdistdefn}
\\
& \subto\;
\sum_{j\in\atoms_2} Z(i,j) \leq \atomwt(i),\;
% \\& \hspace{0.75in}
\sum_{i\in\atoms_1} Z(i,j) \leq \atomwt(j),\; \forall i,j
\end{align*}
\endgroup
Here, the first term is the atom type penalty $\atomtypepen$ which only permits matching
similar atoms, i.e. $\chemmol{C}$ atoms can only be matched to other $\chemmol{C}$ atoms
and not $\chemmol{H}$ or $\chemmol{O}$ atoms.
Accordingly, it is defined as $\atomtypepen(Z) = \langle \atomtypeC, Z \rangle
= \sum_{i\in\atoms_1} \sum_{j\in\atoms_2} \atomtypeC(i,j) Z(i,j)$,
where $Z(i,j) = 0$ if $\atomlabel(i) = \atomlabel(j)$ and $\infty$ otherwise.
The second term is the bond type penalty term, which, similar to $\atomtypepen$,
is given by $\structpen(Z) = \langle \structC, Z \rangle$,
where $\structC(i,j)$ is the penalty for matching unit weight from atom $i\in\atoms_1$ to
atom $j\in\atoms_2$.
We let $\structC(i,j)$ to be the fraction of dissimilar bonds in the union of all bonds;
for example, in Figure~\ref{fig:organicegs},
$\structC(\atomone,\atomtwo) = 3/5$, since, between them they have
one \chemmol{C-H} bond, three \chemmol{C-C}{} bonds, and one \chemmol{C=C} bond,
of which the
the \chemmol{C-H} bond and one \chemmol{C-C} bond are common.
% 
% Since this term accounts for structure, $\structC(i,j)$ is determined by comparing the
% bonds of the atoms $i$ and $j$, and we will consider two options on how this may
% be specified.
% while
% the structural penalty $\structpen$ penalises matching atoms in dissimilar structural
% positions.
If the atom type and bond type penalties are too large or infinite,
we can choose to not match the atoms from
one molecule to another.
However, we will incur a penalty 
via the non-matching penalty term $\nonmatchpen$.
We set this term to be the sum of weights unassigned in both networks,
i.e. 
$\nonmatchpen(Z) =
\sum_{i\in\atoms_1} (\atomwt(i) - \sum_{j\in\atoms_2} Z(i,j)) +
\sum_{j\in\atoms_1} (\atomwt(j) - \sum_{i\in\atoms_1} Z(i,j))$.
For two given molecules $M_1, M_2$, we will denote the resulting dissimilarity measure,
i.e. the solution of~\eqref{eqn:otdistdefn}, by $\otdistsymbol$.
As we will discuss in Appendix ??,~\eqref{eqn:otdistdefn} can be solved via an
optimal transport program.
% Here, $\{w_{1i}\}_{i\in\atoms_1}$, $\{w_{2j}\}_{j\in\atoms_2}$
% are weights which may weight different terms differently.

\textbf{Design choices:}
Finally, let us consider choices for the weights 
$\{\atomwt(a)\}_{a\in\atoms}$ in the matching scheme.
A natural option
here is to let $\atomwt(a)$ be the atomic mass of atom $a$, which assigns more importance
to larger and heavier atoms, which heavily influence the 3D structure of the molecule.
Indeed, the molecular mass (sum of atomic masses)
is commonly used as an indicator of how drug-like a molecule
is, in many metrics including the QED score.
However, lighter atoms may able to influence other important drug-like properties.
For example, the existence of hydroxyl groups (\chemmol{-OH}), is strongly correlated with
solubility in water, since it can function as an electron donor.
The hydrogen atom, which has atomic mass 1, plays a crucial role in this behaviour, and,
setting $\atomwt$ based on the atomic mass would downplay its significance.
In such cases, it is more appropriate to set
$\atomwt(a)=1$ for all atoms, treating them as equal regardless of atomic mass.
In addition to $\otdistsymbol$,
we also consider a normalised version of this dissimilarity,
$\otdistnormsymbol(M_1, M_2) = \otdistsymbol(M_1, M_2) / (\molwt(M_1) + \molwt(M_2))$
where $\molwt(M) = \sum_{a\in A}\atomwt(a)$ is the total weight of a molecule $M=(A,B)$.
Our experience suggested that using $\otdistsymbol$ had a tendency to exaggerate
the dissimilarity between larger molecules, simply because a larger amount of atom weights
needed to be matched.
That said, the size of the molecule affects its drug-like properties (such as its ability
to dock with the target), and $\otdistsymbol$ accounts for the differences between small
and large molecules better than its normalised counterpart.


The two options for the weights $\{\atomwt(a)\}_{a\in\atoms}$ and the two options
for normalisation
gives rise to four different combinations for our dissimilarity measure.
Instead of attempting to find the single best combination, we will instead use a kernel
of the form $\kernel = e^{\sum_i \beta_i d_i}$, where $\{d_i\}_i$ are the
dissimilarity measures obtained for each combination.
An ensemble approach of this form,
allows us to account for all of the factors discussed above when comparing two
molecules.
The $\beta_i$ terms, which affect the relative importance of each measure,
are treated as kernel hyperparameters which can be fitted using maximum likelihood
or posterior sampling techniques~\citep{dragonfly,snoek12practicalBO}.



==> willie_scratch.tex <==
\begin{algorithm}[t]
\small
  \caption{ChemBO}\label{algo:chembo}
  \begin{algorithmic}[1]
  \State \textbf{Input:}   {Number of steps $T$, Initial evaluations $\Dcal_0$}
  \For{$t=1,\ldots,T$}
    \State Infer $\text{GP}(\mu(x), \kappa(x,x') | \Dcal_{t-1})$
    \State $x_t \leftarrow \argmax_{x \in \mathcal{X}} \phi_t$ via \textproc{Acquisition-Optimization}
    \State $m_t \leftarrow \text{Query} x_t$
    \State $\Dcal_t \leftarrow \Dcal_{t-1} \cup \{x_t, m_t\}$
  \Return $m^* \leftarrow \max_{t=1,\ldots,T} m_t$
  \end{algorithmic}
\end{algorithm}
